PKE and ABE with Collusion-Resistant Secure Key Leasing

Secure key leasing (SKL) is an advanced encryption functionality that allows a secret key holder to generate a quantum decryption key and securely lease it to a user. Once the user returns the quantum decryption key (or provides a classical certificate confirming its deletion), they lose their decryption capability. Previous works on public key encryption with SKL (PKE-SKL) have only considered the single-key security model, where the adversary receives at most one quantum decryption key. However, this model does not accurately reflect real-world applications of PKE-SKL. To address this limitation, we introduce collusion-resistant security for PKE-SKL (denoted as PKE-CR-SKL). In this model, the adversary can adaptively obtain multiple quantum decryption keys and access a verification oracle which validates the correctness of queried quantum decryption keys. Importantly, the size of the public key and ciphertexts must remain independent of the total number of generated quantum decryption keys. We present the following constructions: - A PKE-CR-SKL scheme based on the learning with errors (LWE) assumption. - An attribute-based encryption scheme with collusion-resistant SKL (ABE-CR-SKL), also based on the LWE assumption. - An ABE-CR-SKL scheme with classical certificates, relying on multi-input ABE with polynomial arity.

==> def-SKL-RCD.tex <==
% !TEX root = main.tex


\section{Secret-Key Encryption with Collusion-Resistant SKL}

\subsection{Definitions of SKE-CR-SKL}
The syntax of SKE-CR-SKL is defined as follows. 
\begin{definition}[SKE-CR-SKL]
    An SKE-CR-SKL scheme $\SKECRSKL$ is a tuple of five algorithms
$(\Setup,\qKG, \Enc, \qDec, \qVrfy)$. 
Below, let $\cM$  be the message space of $\SKECRSKL$. 
\begin{description}
%\item[$\Setup(1^\secp,1^{\numkey})\ra\msk$:] The setup algorithm takes a security parameter $1^\lambda$ and a collusion bound $1^{\numkey}$, and outputs a master secret key $\msk$.
\item[$\Setup(1^\secp)\ra\msk$:] The setup algorithm takes a
security parameter $1^\lambda$ and outputs a master secret-key
$\msk$.

\item[$\qKG(\msk)\ra(\qdk,\vk,\tk)$:] The key generation algorithm
takes the master secret-key $\msk$ as input. It outputs a decryption
key $\qdk$, a verification key $\vk$, and a testing key
$\tk$.

\item[$\Enc(\msk,\msg)\ra\ct$:] The encryption algorithm takes the
master secret-key $\msk$ and a message $\msg \in \cM$, and outputs a
ciphertext $\ct$.

\item[$\qDec(\qdk,\ct)\ra\widetilde{\msg}$:] The decryption
algorithm takes a decryption key $\qdk$ and a ciphertext $\ct$,
and outputs a value $\widetilde{\msg}$.

%\item[$\qCert(\qfsk)\ra\cert$:] The certification algorithm takes a function decryption key $\qfsk$, and outputs a classical string $\cert$.

\item[$\qVrfy(\vk, \widetilde{\qdk})\ra\top/\bot$:] The verification
    algorithm takes a verification key $\vk$ and a (possibly
    malformed) decryption key $\widetilde{\qdk}$,
and outputs $\top$ or $\bot$.

%\item[$\KeyTest(\tk,\dk)\ra\top/\bot$:] The key testing algorithm takes a key-testing key $\tk$ and a classical decryption key $\dk$, and outputs $\top$ or $\bot$.

\item[Decryption Correctness:] For all $\msg \in \cM$, we have
\begin{align}
\Pr\left[
\qDec(\qdk, \ct) \allowbreak = \msg
\ :
\begin{array}{ll}
\msk\gets\Setup(1^\secp)\\
(\qdk,\vk,\tk)\gets\qKG(\msk)\\
\ct\gets\Enc(\msk,\msg)
\end{array}
\right] 
\ge 1-\negl(\secp).
\end{align}

\item[Verification Correctness:] We have 
\begin{align}
\Pr\left[
\Vrfy(\vk,\qdk)=\top
\ :
\begin{array}{ll}
\msk\gets\Setup(1^\secp)\\
(\qdk,\vk,\tk)\gets\qKG(\msk)\\
\end{array}
\right] 
\ge 1-\negl(\secp).
\end{align}

%\item[Decryption Robustness:]For any $\msg\in\cM$, we have 
%\begin{align}
%\Exp_{
%\begin{scriptsize}
%\begin{array}{lll}
%\msk\gets\Setup(1^\secp)\\
%(\qdk,\vk,\tk)\gets\qKG(\msk)\\
%\ct\gets\Enc(\msk,\msg)
%\end{array}
%\end{scriptsize}
%}
%\left[
%\Pr\left[
%\exists \dk \textrm{~~such that~~}
%\begin{array}{ll}
%\KeyTest(\tk,\dk)=\top\\
%\CDec(\dk,\ct)\ne \msg
%\end{array}
%\right]
%\right]
%=\negl(\secp).
%\end{align}

\end{description}
\end{definition}


\begin{definition}[Classical Decryption Property]
We say that $\SKECRSKL=(\Setup,\qKG,\Enc,\qDec,\qDel, \Vrfy)$ has
the classical decryption property if there exists a deterministic
polynomial time algorithm $\CDec$ such that given $\qdk$ in the
register $\qreg{DK}$ and ciphertext $\ct$, $\qDec$ applies the map
$\ket{u}_{\qreg{DK}}\ket{v}_{\qreg{MSG}}\ra\ket{u}_{\qreg{DK}}\ket{v\oplus\CDec(u,\ct)}_{\qreg{MSG}}$
and outputs the measurement result of the register $\qreg{MSG}$ in
the computational basis, where $\qreg{MSG}$ is initialized to
$\ket{0\cdots0}_{\qreg{MSG}}$.  \end{definition}

\begin{definition}[Key Testability]
We say that an SKE-CR-SKL scheme $\SKECRSKL$ with the classical
decryption property satisfies key testability, if there exists a
classical deterministic algorithm $\KeyTest$ that satisfies the
following conditions:

\begin{itemize}
\item \textbf{Syntax:} $\KeyTest$ takes as input a testing key $\tk$
and a classical string $\dk$ as input. It outputs $0$ or $1$.

\item \textbf{Correctness:} Let $\msk\gets\Setup(1^\secp)$ and
$(\qdk,\vk,\tk)\gets\qKG(\msk)$. We denote the register holding
$\qdk$ as $\qreg{DK}$. Let $\qreg{KT}$ be a register that is
initialized to $\ket{0}_{\qreg{KT}}$. If we apply the map
$\ket{u}_{\qreg{DK}}\ket{\beta}_{\qreg{KT}}\ra\ket{u}_{\qreg{DK}}\ket{\beta\oplus\KeyTest(\tk,u)}_{\qreg{KT}}$
to the registers $\qreg{DK}$ and $\qreg{KT}$ and then measure
$\qreg{KT}$ in the computational basis, we obtain $1$ with
overwhelming probability.

\item \textbf{Security:} Consider the following experiment
$\expb{\SKECRSKL,\qA}{key}{test}(1^\secp)$.

\begin{enumerate}
\item The challenger $\qCh$ runs $\msk\gets\Setup(1^\secp)$ and
initializes $\qA$ with input $\msk$. 

\item $\qA$ requests $q$ decryption keys for some polynomial $q$.
$\qCh$ generates $(\qdk_i,\vk_i,\tk_i)\gets\qKG(\msk)$
for every $i\in[q]$ and sends $(\qdk_i,\vk_i,\tk_i)_{i\in[q]}$ to
$\qA$.

\item $\qA$ sends $(k, \dk, \msg)$ to $\qCh$, where $k$ is
an index, $\dk$ is a classical string and $\msg$ is a message.
$\qCh$ generates $\ct\gets\Enc(\msk,\msg)$. $\qCh$ outputs $\top$ if
$\KeyTest(\tk_k,\dk)=1$ and $\CDec(\dk,\ct)\ne\msg$.
Otherwise, $\qCh$ outputs $\bot$.
\end{enumerate}

For all QPT $\qA$, the following must hold:

\begin{align}
\advb{\SKECRSKL,\qA}{key}{test}(1^\secp) \seteq
\Pr[\expb{\SKECRSKL,\qA}{key}{test}(1^\secp) \ra \top] \le
\negl(\secp).
\end{align} 
\end{itemize}
\end{definition}

\begin{definition}[OT-IND-KLA Security]\label{def:OT-IND-CPA_SKECRSKL}
%\takashi{Renamed from lessor security to IND-CPA security. (Alternatively, should we call it something like IND-KLA (Key Leasing Attack)?)}
We say that an SKE-CR-SKL scheme with key testability $\SKECRSKL$
is OT-IND-KLA secure, if it satisfies
the following requirement, formalized by the experiment
$\expc{\SKECRSKL,\qA}{ot}{ind}{kla}(1^\secp,\coin)$ between an
adversary $\qA$ and a challenger $\qCh$:

\begin{enumerate}
\item $\qCh$ runs $\msk\gets\Setup(1^\secp)$ and initializes
$\qA$ with the security parameter $1^\secp$.

\item $\qA$ requests $q$ decryption keys for some polynomial $q$.
The challenger generates $(\qdk_i,\vk_i,\tk_i)\gets\qKG(\msk)$
for every $i\in[q]$ and sends $(\qdk_i,\tk_i)_{i\in[q]}$ to $\qA$.

\item $\qA$ can get access to the following (stateful) verification
oracle $\Oracle{\qVrfy}$ where $V_i$ is initialized to be $\bot$:

\begin{description}
\item[ $\Oracle{\qVrfy}(i, \widetilde{\qdk})$:] It runs $d \gets
\Vrfy(\vk_i, \widetilde{\qdk})$ and returns $d$.  

If $V_i=\bot$ and $d=\top$, it updates $V_i\seteq \top$. 
               %\takashi{changed the way of explaining update to better match that for ABE/FE.}
               %and updates $V\seteq \returned$ if $d=\top$. 
\end{description}
\item $\qA$ sends $(\msg_0^*,\msg_1^*)\in \cM^2$ to the challenger.
If $V_i=\bot$ for some $i\in[q]$, $\qCh$ outputs
$0$ as the final output of this experiment. Otherwise, $\qCh$
generates $\ct^*\la\Enc(\msk,\msg_\coin^*)$ and sends
$\ct^*$ to $\qA$.

\item $\qA$ outputs a guess $\coin^\prime$ for $\coin$.
$\qCh$ outputs $\coin'$ as the final output of the
experiment.
\end{enumerate}

For all QPT $\qA$, it holds that:
\begin{align}
\advc{\SKECRSKL,\qA}{ot}{ind}{kla}(1^\secp) \seteq \abs{\Pr[\expc{\SKECRSKL,\qA}{ot}{ind}{kla} (1^\secp,0) \ra 1] - \Pr[\expc{\SKECRSKL,\qA}{ot}{ind}{kla} (1^\secp,1) \ra 1] }\leq \negl(\secp).
\end{align} 
\end{definition}

\subsection{Definitions of
SKE-CR\textsuperscript{2}-SKL}\label{def:ske-cr2}
The syntax of SKE-CR\textsuperscript{2}-SKL is defined as follows. 
\begin{definition}[SKE-CR\textsuperscript{2}-SKL]
An SKE-CR\textsuperscript{2}-SKL scheme $\SKECRCRSKL$ is a tuple of
six algorithms $(\Setup,\qKG, \Enc, \qDec, \allowbreak \qDel, \Vrfy)$. 
Below, let $\cM$  be the message space of $\SKECRCRSKL$. 
\begin{description}
\item[$\Setup(1^\secp)\ra\msk$:] The setup algorithm takes a
security parameter $1^\lambda$ and outputs a master secret-key
$\msk$.

\item[$\qKG(\msk)\ra(\qdk,\vk)$:] The key generation algorithm
takes the master secret-key $\msk$ as input. It outputs a decryption
key $\qdk$ and a certificate verification key $\vk$.

\item[$\Enc(\msk,\msg)\ra\ct$:] The encryption algorithm takes the
master secret-key $\msk$ and a message $\msg \in \cM$, and outputs a
ciphertext $\ct$.

\item[$\qDec(\qdk,\ct)\ra\widetilde{\msg}$:] The decryption
algorithm takes a decryption key $\qdk$ and a ciphertext $\ct$,
and outputs a value $\widetilde{\msg}$.

%\item[$\qCert(\qfsk)\ra\cert$:] The certification algorithm takes a function decryption key $\qfsk$, and outputs a classical string $\cert$.

\item[$\qDel(\qdk)\ra\cert$:] The decryption
algorithm takes a decryption key $\qdk$ and outputs a
certificate $\cert$.

\item[$\Vrfy(\vk, \cert')\ra\top/\bot$:] The verification
algorithm takes a verification key $\vk$ and a certificate $\cert'$
, and outputs $\top$ or $\bot$.

\item[Decryption Correctness:] For all $\msg \in \cM$, we have
\begin{align}
\Pr\left[
\qDec(\qdk, \ct) \allowbreak = \msg
\ :
\begin{array}{ll}
\msk\gets\Setup(1^\secp)\\
(\qdk,\vk)\gets\qKG(\msk)\\
\ct\gets\Enc(\msk,\msg)
\end{array}
\right] 
\ge 1-\negl(\secp).
\end{align}

\item[Verification Correctness:] We have 
\begin{align}
\Pr\left[
\Vrfy(\vk,\cert)=\top
\ :
\begin{array}{ll}
\msk\gets\Setup(1^\secp)\\
(\qdk,\vk)\gets\qKG(\msk)\\
\cert \gets\qDel(\qdk)
\end{array}
\right] 
\ge 1-\negl(\secp).
\end{align}

%\item[Decryption Robustness:]For any $\msg\in\cM$, we have 
%\begin{align}
%\Exp_{
%\begin{scriptsize}
%\begin{array}{lll}
%\msk\gets\Setup(1^\secp)\\
%(\qdk,\vk,\tk)\gets\qKG(\msk)\\
%\ct\gets\Enc(\msk,\msg)
%\end{array}
%\end{scriptsize}
%}
%\left[
%\Pr\left[
%\exists \dk \textrm{~~such that~~}
%\begin{array}{ll}
%\KeyTest(\tk,\dk)=\top\\
%\CDec(\dk,\ct)\ne \msg
%\end{array}
%\right]
%\right]
%=\negl(\secp).
%\end{align}

\end{description}
\end{definition}


\begin{description}
\item[IND-KLA Security:] The IND-KLA Security of an
SKE-CR\textsuperscript{2}-SKL scheme is defined in the same way as
the OT-IND-KLA Security (Definition \ref{def:OT-IND-CPA_SKECRSKL})
of an SKE-CR-SKL scheme, except that throughout the experiment,
$\qA$ receives access to the following oracle:

\begin{description}
\item[ $\Oracle{\Enc}(\msg)$:] It runs $\ct \gets \Enc(\msk,
\msg)$ and returns $\ct$.  

\end{description}

Furthermore, the access to the oracle $\Oracle{\qVrfy}$ is replaced
with access to the following oracle:
\begin{description}
\item[ $\Oracle{\Vrfy}(i, \textcolor{black}{\cert})$:] It runs $d
\gets \Vrfy(\vk_i,\textcolor{black}{\cert})$ and returns $d$.  

If $V_i=\bot$ and $d=\top$, it updates $V_i\seteq \top$. 
\end{description}
\end{description}

==> obsolete_files/const-PKE-CR2-SKL.tex <==
\section{Construction of \tPKECRCRSKL}

\begin{comment}
\nikhil{They seem to build (Adaptive-Secure) (Multi-Input) (Predicate) Encryption for polynomial arity for P. All three prefixes are stronger than what we need, which is (Selective-Secure) (Multi-Key) (Attribute-Based) Encryption.}
\end{comment}

The building blocks of the construction
$\PKECRCRSKL = \PKECRCRSKL.(\Setup, \qKG, \Enc,$ 
$\qDec, \qDel, \Vrfy)$ are as follows:

\begin{itemize}
\item Multi-Key (Ciphertext-Policy) ABE Scheme $\MKABE =
\MKABE.(\Setup, \KG, \Enc, \Dec)$ for the following relation:

\begin{description}
\item[$R(x, u_1, \cdots, u_\ell)$:] Let $x$ be
interpreted as an $\ell$-input circuit.
\begin{itemize}
\item If $x\big(u_1, \cdots, u_\ell) = \bot$, output $0$
(decryptable).
\item Else, output $1$.
\end{itemize}
\end{description}

\item Compute-and-Compare Obfuscation $\CCObf$ with the simulator
$\CCSim$.

\item Random Oracle $H$.

\item Secret-Key Encryption Scheme $\SKE = \SKE.(\Enc,
\Dec)$.
\end{itemize}

The construction is described as follows:

\begin{description}
\item[$\PKECRCRSKL.\Setup(1^\secp)$:] $ $
\begin{itemize}
\item Generate $(\abe.\pk,\abe.\msk_1, \cdots, \abe.\msk_\ell)\gets\MKABE.\Setup(1^\secp)$.
\item Generate $\ske.\sk\gets \bit^\secp$.
\item Output $\ek\seteq\abe.\pk$ and
    $\msk\seteq(\{\abe.\msk_i\}_{i\in[\ell]},\ske.\sk)$.
\end{itemize}

\item[$\PKECRCRSKL.\qKG(\msk)$:] $ $
\begin{itemize}
\item Parse $\msk=(\abe.\msk,\ske.\sk)$.
\item Sample random $r_1, \cdots, r_\ell$ such that $r_1 \xor \cdots
\xor r_\ell = 0^{\secp}$.
\item Sample a random value $y \gets \bit^\secp$.

\item For each $i \in [\ell]$, compute the following:
\begin{itemize}
\item Sample $(x_0^i, x_1^i) \leftarrow
\bit^\secp \times \bit^\secp$.

\item Compute $\ske.\ct_i = \SKE.\Enc(\ske.\sk, H(x_0^i) \xor r_i,
H(x_1^i) \xor r_i)$.

\item For each $b \in \bit$, compute $\abe.\dk_b^i =
\MKABE.\KG(\abe.\msk_i, y \| x_b^i \| \ske.\ct_i)_\qreg{ABE_i}$.

\item
Prepare the following state $\rho_i$:
$$\ket{0}_{\qreg{A_i}}\ket{x_0^i}_{\qreg{B_i}}\ket{\abe.\dk_0^i}_\qreg{ABE_i} +
\ket{1}_{\qreg{A_i}}\ket{x_1^i
}_{\qreg{B_i}}\ket{\abe.\dk_1^i}_\qreg{ABE_i}.$$


\end{itemize}
\item Output $\qdk = (\rho_i)_{i \in [\ell]}$ and $\vk =
\big((\abe.\dk_0^i \xor \abe.\dk_1^i)_{i \in [\ell]}, (x_0^i
\xor x_1^i)_{i \in [\ell]}\big)$.
\end{itemize}

\item[$\PKECRCRSKL.\Enc(\ek,\msg)$:] $ $
\begin{itemize}
\item Parse $\ek=\abe.\pk$.
\item Generate $\tlC\gets\CCSim(1^\secp)$.
\item Let $B[\tlC]$ be a circuit defined as follows:
\begin{description}
\item[$B{[}\tlC{]}(u_1, \cdots, u_\ell)$:] $ $
\begin{itemize}
\item For each $i \in [\ell]$, parse $u_i = y_i \| z_i$.
\item Output $\bot$ if $\big(\tlC(z_1 \| \cdots \| z_\ell) =
\bot\big) \land \big(y_1 = \cdots = y_\ell\big)$.
\item Otherwise, output $0$.
\end{itemize}
\end{description}

\item Generate $\abe.\ct\gets\MKABE.\Enc(\abe.\pk,B[\tlC],\msg)$.
\item Output $\ct\seteq\abe.\ct$.
\end{itemize}

\item[$\PKECRCRSKL.\qDec(\qdk,\ct)$:] $ $
\begin{itemize}
\item Parse $\ct=\abe.\ct$ and $\qdk = (\rho_i)_{i \in [\ell]}$. Let
the register holding $\rho_i$ be denoted as $\qreg{A_i} \otimes
\qreg{B_i} \otimes \qreg{ABE_i}$. 
\item Prepare a register $\qreg{MSG}$ that is initialized to
$\ket{0\cdots0}_{\qreg{MSG}}$.

\item Apply the map:
$\bigotimes_{i=1}^{\ell}\ket{v_i}_{\qreg{ABE_i}}\otimes
\ket{w}_{\qreg{MSG}}\ra
\bigotimes_{i=1}^{\ell}\ket{v_i}_{\qreg{ABE_i}}\otimes\ket{w\oplus\MKABE.\Dec(\abe.\ct, v_1, \cdots, v_l)}_{\qreg{MSG}}$ to the registers
$\bigotimes_{i=1}^\ell\qreg{ABE_i}$ and $\qreg{MSG}$.
\item Measure the register $\qreg{MSG}$ in the computational basis
and output the result $\msg^\prime$.
\end{itemize}

\item[$\PKECRCRSKL.\qDel(\qdk)$:] $ $
\begin{itemize}
\item Parse $\qdk = (\rho_i)_{i \in [\ell]}$. Let the register 
holding $\rho_i$ be denoted as $\qreg{A_i} \otimes \qreg{B_i}
\otimes \qreg{ABE_i}$.
\item For each $i \in [\ell]$, measure the registers $\qreg{A_i}$,
$\qreg{B_i}$, and $\qreg{ABE_i}$ in the Hadamard basis to
obtain outcomes $c_i, d_i$, and $e_i$.
\item Output $\cert = (c_i, d_i, e_i)_{i \in [\ell]}$.
\end{itemize}

\item[$\PKECRCRSKL.\Vrfy(\vk, \cert')$:] $ $
\begin{itemize}
\item Parse $\vk =
\big((\abe.\dk_0^i \xor \abe.\dk_1^i)_{i \in [\ell]}, (x_0^i \xor
x_1^i)_{i \in [\ell]}\big)$ and $\cert' = (c_i, d_i, e_i)_{i \in
[\ell]}$.

\item For each $i \in [\ell]$, check if $c_i = \big\langle d_i
\| e_i, (x_0^i \xor x_1^i) \| (\abe.\dk_0^i \xor
\abe.\dk_1^i)\big\rangle$. Output $\top$ if the check passes for all
$i \in [\ell]$. Else, output $\bot$.
\end{itemize}
\end{description}

\paragraph{Security of Building Block:}
Consider the following experiment $\mathsf{Exp}_\qA(1^\secp,
\coin)$:

\begin{enumerate}
\item $\qA$ sends $(m_0, m_1) \in \bit^\secp \times \bit^\secp$ to
$\qCh$ and $q = \poly(\secp)$.

\item $\qCh$ chooses $\sk \gets \bit^\secp$.

\item For each $j \in [q]$, $\qCh$ computes the following:
\begin{itemize}
\item Sample random $r_1^j, \cdots, r_\ell^j$ such that $r_1^j
\xor \cdots \xor r_\ell^j = m_\coin$.

\item For each $i \in [\ell]$, sample $x_0^{i, j}, x_1^{i, j} \gets
\bit^\secp \times \bit^\secp$ and prepare the following state:

$$\rho_i^j = \ket{0}\ket{x_0^{i,j}} + \ket{1}\ket{x_1^{i, j}}$$

$$\ct_i^j \gets \SKE.\Enc\Big(\sk, H(x_0^{i,j}) \xor r_i^j,
H(x_1^{i,j}) \xor r_i^j\Big)$$

\item Set $\rho^j = (\rho^j_i)_{i \in [\ell]}$ and $\ct^j =
(\ct_i^j)_{i \in [\ell]}$.
\end{itemize}

\item $\qCh$ sends $(\rho^j, \ct^j)_{j \in [q]}$ to $\qA$.

\item For each $j \in [q]$, $\qA$ sends
$(c_i^j, d_i^j)_{i \in [\ell]}$ to $\qCh$.

\item For each $(i, j) \in [\ell]\times[q]$, $\qCh$ checks if
$d_i^j\cdot(x^{i,j}_0 \xor x^{i,j}_1) = c_i^j$ holds. If all checks
pass, it sends $\sk$ to $\qA$. Else, it outputs $\perp$.

\item $\qA$ outputs a guess $\coin'$. $\qCh$ outputs $\coin'$ as the
final output of the experiment.
\end{enumerate}

We have the following security requirement:

$$\mathsf{Adv}_\qA(1^\secp) \seteq \Big\lvert
\Pr[\mathsf{Exp}_\qA(1^\secp, 0) \ra 1] -
\Pr[\mathsf{Exp}_\qA(1^\secp, 1) \ra 1]\Big\rvert \le \negl(\secp)$$

\paragraph{Security Proof of \tPKECRCRSKL:}

Let $\qA$ be an adversary for the IND-KLA security of $\PKECRSKL$.
We consider the following sequence of experiments.
\begin{description}
\item[$\hybi{0}^\coin$:] This is
$\expb{\PKECRCRSKL,\qA}{ind}{kla}(1^\secp,\coin)$.

\item[$\hybi{1}^\coin$:] This is the same as $\hybi{0}^\coin$ except
that instead of $\tlC$ being generated as $\tlC \gets
\CCSim(1^\secp)$, it is generated as follows:

$$\tlC \gets \CCObf(P[\sk], \lock, 0^\secp)$$ where $P[\sk]$ is a
circuit defined as follows:

\begin{description}
\item[$P{[}\sk{]}(z)$:] $ $
\begin{itemize}
\item Parse $z = z_1 \| \cdots \| z_\ell$.
\item For each $i \in [\ell]$, do the following:
\begin{itemize}
\item Parse $z_i = x^i_b \| \ske.\ct_i$.
\item Compute $r_i = \SKE.\Dec(\sk, \ske.\ct_i) \xor H(x_b^i)$.
\end{itemize}
\item Output $r_1 \xor \cdots \xor r_\ell$.
\end{itemize}
\end{description}

Notice that $\qA$'s view and $P[\sk]$ are independent of $\lock$.
Hence, from the security of compute-and-compare obfuscation, we have
that $\Hyb_1^\coin \approx \Hyb_0^\coin$.

\item[$\hybi{2}^\coin$:] This is the same as $\Hyb_1^\coin$ except
that all the decryption keys $\qdk_1, \cdots, \qdk_q$ are generated
with the following change: $r_1, \cdots, r_\ell$ are chosen at
random such that $r_1 \xor \cdots \xor r_\ell = \lock$. Conditioned
on every deletion check passing, this switch is undetectable by the
security of the building block. Hence, we have $\Hyb_2^\coin \approx
\Hyb_1^\coin$. 

\nikhil{Need to account for oracle queries using some kind of
key-testability style arguments.}

\item[$\hybi{3}^\coin$:] This is the same as $\Hyb_2^\coin$ except
that $\abe.\ct^\star$ is generated as $\abe.\ct^\star \gets
\MKABE.\Enc(\abe.\pk, B[\tlC], 0^\secp)$.
Since $P[\sk](z)$ outputs $r_1 \xor \cdots \xor r_\ell = \lock$,
$\tlC$ outputs $0^\secp$ instead of $\bot$. Now, by the
security of MK-ABE, $\qA$ can distinguish between $\Hyb_3^\coin$
and $\Hyb_2^\coin$ only if it has some set of $\ell$ keys satisfying
both conditions checked by the ciphertext attribute $B[\tlC]$.
However, it is easy to see that for any set of $\ell$ keys, at least
one of the conditions is false.

\end{description}

==> preamble_newtheorem.tex <==
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}{Lemma} 
\newtheorem{claim}{Claim}  
\newtheorem{proposition}{Proposition} 
\newtheorem{definition}{Definition}  
\newtheorem{fact}{Fact}  
\newtheorem{remark}{Remark}  
%\newtheorem{proof}{Proof}  % Already defined by ``amsthm" package. Only include it when ``amsthm" is not used.
\newtheorem{corollary}{Corollary} 

==> preamble_usepackages_ex.tex <==

\usepackage[%
%  dvipdfmx, 
  colorlinks=true,
  citecolor=darkgreen,
  linkcolor=darkblue,
  urlcolor=darkblue,
  pagebackref=true
]{hyperref}

\usepackage{amsmath, amsfonts, amssymb, mathtools,amscd}
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}

\usepackage{lmodern}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

\usepackage{etex}

\usepackage{arydshln} % In order to use \hdashline
\usepackage{url}
\usepackage{ifthen}
\usepackage{bm}
\usepackage{multirow}
\usepackage[dvips]{graphicx}
\usepackage[usenames]{color}
\usepackage{xcolor,colortbl} % Leave out in case the usepackage cannot be found. Not critical
\usepackage{threeparttable}
\usepackage{comment}
\usepackage{paralist,verbatim}
\usepackage{cases}
\usepackage{booktabs}
\usepackage{braket}
\usepackage{cancel} 
\usepackage{ascmac} 
\usepackage{framed}
% \usepackage{authblk}
\usepackage{pifont}
\usepackage{physics}
%\usepackage[dvipsnames]{xcolor}
\definecolor{darkblue}{rgb}{0,0,0.6}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{maroon}{rgb}{0.5,0.1,0.1}
\definecolor{dpurple}{rgb}{0.2,0,0.65}
\definecolor{chocolate}{rgb}{0.8,0.4,0.1}

\usepackage[capitalise,noabbrev]{cleveref}
\usepackage[absolute]{textpos}
\usepackage[final]{microtype}
\usepackage[absolute]{textpos}
\usepackage{everypage}
\usepackage{autonum}

\usepackage{dsfont}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\ifnum\submission=1
\renewcommand*{\backref}[1]{}
\def\notxfont{1}
\pagestyle{plain}
\else
\fi


\ifnum\llncs=1
\renewcommand{\subparagraph}{\paragraph}
\else
\ifnum\notxfont=1
\else
\usepackage{mathpazo}
\usepackage{newtxtext}
\usepackage{helvet}
\fi
\fi


\newcommand{\heading}[1]{{\vspace{1ex}\noindent\sc{#1}}}

%%%%%%%%%%%%%%% Proof environment in non-LNCS style %%%%%%%%%%%%%%%%%%%
\newtheoremstyle{thicktheorem}%
{\topsep}
{\topsep}
{\itshape}{}%
{\bfseries}%
{.}
{ }%
{\thmname{#1}\thmnumber{ #2}%
		\thmnote{ (#3)}%
}

\newtheoremstyle{remark}%name
{\topsep}
{\topsep}
	{}%body font
	{}%indent amount
	{}%theorem head font
	{.}%punctuation after theorem head
	{ }%space after theorem head
	{\textit{\thmname{#1}}\thmnumber{ #2}%theorem head specs
			\thmnote{ (#3)}%
	}

\ifnum\llncs=0
	\theoremstyle{thicktheorem}
	\newtheorem{theorem}{Theorem}[section]
	\newtheorem{lemma}[theorem]{Lemma}
	\newtheorem{corollary}[theorem]{Corollary}
	\newtheorem{proposition}[theorem]{Proposition}
	\newtheorem{definition}[theorem]{Definition}

	\theoremstyle{remark}
	\newtheorem{claim}[theorem]{Claim}
	\newtheorem{remark}[theorem]{Remark}
	\newtheorem{example}[theorem]{Example}
	\newtheorem{note}[theorem]{Note}
	\newtheorem{conjecture}[theorem]{Conjecture}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


	\crefname{theorem}{Theorem}{Theorems}
	\crefname{assumption}{Assumption}{Assumptions}
	\crefname{construction}{Construction}{Constructions}
	\crefname{corollary}{Corollary}{Corollaries}
	\crefname{conjecture}{Conjecture}{Conjectures}
	\crefname{definition}{Definition}{Definitions}
	\crefname{exmaple}{Example}{Examples}
	\crefname{experiment}{Experiment}{Experiments}
	\crefname{counterexample}{Counterexample}{Counterexamples}
	\crefname{lemma}{Lemma}{Lemmata}
	\crefname{observation}{Observation}{Observations}
	\crefname{proposition}{Proposition}{Propositions}
	\crefname{remark}{Remark}{Remarks}
	\crefname{claim}{Claim}{Claims}
	\crefname{fact}{Fact}{Facts}
	\crefname{note}{Note}{Notes}

\ifnum\llncs=1
 \crefname{appendix}{App.}{Appendices}
 \crefname{section}{Sec.}{Sections}
\else
\fi

\ifnum\llncs=1
%\thispagestyle{empty}
\pagestyle{plain}
\renewcommand*{\backref}[1]{}
\else
	\renewcommand*{\backref}[1]{(Cited on page~#1.)}
	\ifnum\notxfont=1
	\else
		\usepackage{newtxtext}
	\fi
\fi


==> todo.tex <==
\section{To Do}

\subsection*{\nikhil{}}

\begin{enumerate}
\item $[\;]$ Formal Details of q-Security of ABE.
\item $[\;]$ Multi-Input ABE Preliminaries (incl AKY Theorem).
\item $[\;]$ Elaborate MI-ABE Reduction in
    PKE-CR\textsuperscript{2}-SKL Proof.
\item $[\;]$ Write SKE-CR\textsuperscript{2}-SKL Para (on
Construction) and Proof (justify based on PKE proof and AKY).
\item $[\;]$ Proofread ABE-SKL Section.
\end{enumerate}
